On Data Augmentation and Adversarial Risk: An Empirical Analysis

Data augmentation techniques have become standard practice in deep learning, as it has been shown to greatly improve the generalisation abilities of models. These techniques rely on different ideas such as invariance-preserving transformations (e.g, expert-defined augmentation), statistical heuristics (e.g, Mixup), and learning the data distribution (e.g, GANs). However, in the adversarial settings it remains unclear under what conditions such data augmentation methods reduce or even worsen the misclassification risk. In this paper, we therefore analyse the effect of different data augmentation techniques on the adversarial risk by three measures: (a) the well-known risk under adversarial attacks, (b) a new measure of prediction-change stress based on the Laplacian operator, and (c) the influence of training examples on prediction. The results of our empirical analysis disprove the hypothesis that an improvement in the classification performance induced by a data augmentation is always accompanied by an improvement in the risk under adversarial attack. Further, our results reveal that the augmented data has more influence than the non-augmented data, on the resulting models. Taken together, our results suggest that general-purpose data augmentations that do not take into the account the characteristics of the data and the task, must be applied with care.

==> remaining_tasks.tex <==
\section*{Remaining tasks}
\hamid{This is to report what tasks are still remaining for the full paper submission.
If you want to contribute, please take a look at the following list, 
and choose one (or more) of the available open tasks, and \textbf{add your name to that task in the `people working on it:' section.}}

\hamid{\textbf{Also please use OVERLEAF COMMENTS to leave feedback, as using latext comments increases the length of the paper, and will be problematic as I am trying to meet the maximum length.
Also using the `resolve option' makes it easier to track the changes.}
}

\begin{enumerate}
    \item Abstract: \finished{}, \proofread{}. (people working on it: \hamid{}, \yourname{Gerhard, Bernhard, and Werner could help here.})
    \item Intro section: \finished{}, \proofread{}. (people working on it: \hamid{}, \gerhard{},  \yourname{Gerhard, Bernhard, and Werner could help here.})
    \item Definitions: \finished{}. (people working on it: \werner{}, \bernhard{}, \michal{})
    \item Empirical evaluations:
    \begin{enumerate}
    \item Goals and Questions: \finished{}, \proofread{}. (people working on it: \hamid{},  \gerhard{})
    \item Experimental setup:\finished{}, \proofread{}. (people working on it: \hamid{},  )
    \item Classification Error and Risk Under Attack results:\finished{}, \proofread{}. (people working on it: \hamid{},  )
    \item Prediction-Change Stress results: \finished{}, \proofread{}. (people working on it:  \khaled{khaled},\hamid{}, \yourname{Hamid and Werner could help here.})
    \item Influence scores results:\finished{}, \proofread{}. (people working on it: \paul{},\hamid{}, \yourname{Hamid and Werner could help here.})
  \end{enumerate}
  \item Conclusion: \finished{} \proofread{}. (people working on it:\hamid{} \yourname{Gerhard and Bernhard could help here.} )
  \item Broader impact: \finished{} \proofread{}. (people working on it:\gerhard{} \yourname{Gerhard and Bernhard could help here.} )
   \item Appendix (deadline for supplementary material is Jun 11).
     \begin{enumerate}
     \item additional Prediction-Change Stress results: \notwritten{}.(people working on it: \khaled{khaled},   )
     \item additional Influence scores results: \notwritten{}.(people working on it: \hamid{}, \paul{}, )
     \item experiment setup \notwritten{}.(people working on it: \hamid{})
    \end{enumerate}
    \item  proofreading the full paper: \notdone{} (people working on it:  \yourname{All co-authors could help here.})
\end{enumerate}
Also please have a look at the following material:
\begin{enumerate}
\item FAQ:
\url{https://neurips.cc/Conferences/2020/PaperInformation/NeurIPS-FAQ}

important from FAQ:
\textbf{Q: What do my co-authors and I need to complete before the co-author registration deadline? 
A: Before the paper submission deadline, the submitting author needs to enter the co-author list making sure that email addresses used to identify co-authors match their CMT email addresses. Note that the author list and email addresses cannot be changed after the paper submission deadline. Then, before the co-author registration deadline, every co-author needs to login and fill out the user-information form on the NeurIPS2020 CMT site to enable a smooth review process without conflicts of interest. The form will ask each co-author to enter a) the list of her/his email addresses used for publication and reviewing, b) the list of URL to relevant papers describing her/his area of expertise, c) domain and personal conflicts of interest, and information useful to assess their reviewing experience.}

\item CFP:
\url{https://neurips.cc/Conferences/2020/CallForPapers}

\item `A Note for Submitting Authors' from NeurIPS organizers:

\url{https://medium.com/@NeurIPSConf/a-note-for-submitting-authors-48cebfebae82}
\item `The reviewing process in NeurIPS2020' from NeurIPS organizers:

\url{https://www.youtube.com/watch?v=361h6lHZGDg}
\item Suggestions about how to write `The Broader Impact' section:
\begin{enumerate}
    \item \url{https://medium.com/@BrentH/suggestions-for-writing-neurips-2020-broader-impacts-statements-121da1b765bf}
    \item \url{https://medium.com/@operations_18894/a-guide-to-writing-the-neurips-impact-statement-4293b723f832}
\end{enumerate}



\end{enumerate}

\clearpage\null%\newpage
